Small-Scale Testbed for Evaluating C-V2X Applications on 5G Cellular Networks

In this work, we present a small-scale testbed for evaluating the real-life performance of cellular V2X (C-V2X) applications on 5G cellular networks. Despite the growing interest and rapid technology development for V2X applications, researchers still struggle to prototype V2X applications with real wireless networks, hardware, and software in the loop in a controlled environment. To help alleviate this challenge, we present a testbed designed to accelerate development and evaluation of C-V2X applications on 5G cellular networks. By including a small-scale vehicle platform into the testbed design, we significantly reduce the time and effort required to test new C-V2X applications on 5G cellular networks. With a focus around the integration of small-scale vehicle platforms, we detail the design decisions behind the full software and hardware setup of commonly needed intelligent transport system agents (e.g. sensors, servers, vehicles). Moreover, to showcase the testbed's capability to produce industrially-relevant, real world performance evaluations, we present an evaluation of a simple test case inspired from shared situational awareness. Finally, we discuss the upcoming use of the testbed for evaluating 5G cellular network-based shared situational awareness and other C-V2X applications.

==> src/4_case.tex <==
% Shared Situational Awareness

Many industries divide CAV framework functionality into various layers, i.e. sensing, localization, perception, situational awareness, planning, and control. The Situational awareness of the vehicle is ability to perceive and comprehend a traffic situation and to estimate the state of the vehicles and road-users in the surrounding of the ego-vehicle. This situational awareness layer relies on the perception layer of the vehicle, which provides information about the dynamic objects in the near surrounding of the ego-vehicle. When a CAV is located in any urban scenario, the field-of-view (FOV) of the CAV is severely affected by occlusions which leads to limited information about the surroundings and affects situational awareness of the CAV. 

In this case study we refer to~\cite{Narri_Alanwar_2023}, where the authors have implemented shared situational awareness framework, with an objective to improve situational awareness of the ego-vehicle using V2X communication. In this cited paper, a simple urban scenario is considered, where the FOV of the ego-vehicle has an occlusion created by a parked vehicle. But this occluded region is visible for two other connected V2X units in the near surrounding. The connected V2X unit share their perception data i.e. respect to their location, with the ego-vehicle using ITS-G5 access layer specification published by the European Telecommunications Standards Institute (ETSI)~\cite{etsi_its_g5}. ITS-G5 is a European standard for vehicular communication based on IEEE 802.11 standards for its lower layers. In the cited work, the authors utilize the standardized  Collaborative Perception Message (CPM)~\cite{ETSI_TR_103_562}.

In these standard, a general message structure consists of Management Container (MC), Station Data Container (SDC), Sensor Information Container (SIC), Perceived Object Container (POC), and Free Space Addendum (FSA). The shared situational awareness framework relies on MC, SDC and POC~\cite{Narri_Alanwar_2023}, where MC provides basic information about the originating ITS-S (Intelligent Transport System-Station), which includes the station type and reference position in the global coordinates. The SDC provides more specific information about the originating ITS-S in addition to the common information provided by the MC. The data received from the perception module of SV or RSU is populated into the POC of the CPM. The POC enables a detailed description of the dynamic state and properties of a detected object.

In this cited work, the tests perform have a communication frequency of 5.900 GHz. The range was more than 1000 meters, as the tests are performed in an open field. Each message is sent and receive at a frequency of 10 Hz. The total payload of each message was 156 bytes and each message consists of MC, SIC and POC. In each message there were five POCs, which had a payload of 78 bytes. According to IEEE 802.11 standards, the ITS-G5 network has a limitation to send each message with a maximum payload of 1500 bytes.

In this work, we are interested in evaluating the messaging capabilities within the 5G network to understand how a 5G-based shared situational awareness system could be designed. Since 5G networks have different bandwidth limitations and different features for prioritizing messages in the network, we set up a test case where we evaluate the testbed's performance with varying network loads, message sizes, and frequencies. Moreover, since safety critical data is being communicated, it's of interest to understand the effects of network traffic overloading and handovers on the messaging between agents.


==> src/table.tex <==
\begin{table}[!ht]
    \centering
    % \renewcommand{\arraystretch}{2}
    \begin{tabular}{c>{\centering\arraybackslash}m{2.2cm} >{\centering\arraybackslash}m{2.6cm} >{\centering\arraybackslash}m{1cm} >{\centering\arraybackslash}m{1cm}}
        \hline
        & \textbf{\begin{tabular}[c]{@{}c@{}}Network\\ Config.\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Background Load\\ Uplink - Downlink\\ {[Mbps]}\end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Message\\ Size\\ {[kB]}\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Message\\ Frequency\\ {[Hz]}\end{tabular}} \\ 
        \hline \hline
        \multirow{8}{*}{\rotatebox[origin=c]{90}{Nominal}} & \multirow{4}{*}{BL} & \multirow{2}{*}{No Load - No Load}& 1 & 10 / 20 \\
        & & & 10 & 10 / 20 \\ 
        \cline{3-5} 
        & & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}1 x 5 - 1 x 110\end{tabular}} & 1 & 10 / 20 \\
        & & & 10 & 10 / 20 \\ 
        \cline{2-5} 
        & \multirow{4}{*}{AP} & \multirow{2}{*}{No Load - No Load} & 1 & 10 / 20 \\
        & & & 10 & 10 / 20 \\ 
        \cline{3-5} 
        & & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}1 x 5 - 1 x 110\end{tabular}} & 1 & 10 / 20 \\
        & & & 10 & 10 / 20 \\ 
        \hline
        \multirow{4}{*}{\rotatebox[origin=c]{90}{Overload}} & \multirow{2}{*}{BL} & 1 x 40 - No Load & 10 & 20 \\
        & & 2 x 40 - No Load & 10 & 20 \\ 
        \cline{2-5} 
        & \multirow{2}{*}{AP} & 1 x 40 - No Load & 10 & 20 \\
        & & 2 x 40 - No Load & 10 & 20 \\ 
        \hline
        \rotatebox[origin=c]{90}{ Mobility } & BL & No Load - No Load & 10 & 20 \\ 
        \hline
    \end{tabular}
    \caption{Combinations of network configurations, background load, message sizes, and frequencies in the presented test case.}
    \label{tab:combinations_experiments}
\end{table}
